Towards Continuous Assurance Case Creation for ADS with the Evidential Tool Bus

An assurance case has become an integral component for the certification of safety-critical systems. While manually defining assurance case patterns can be not avoided, system-specific instantiations of assurance case patterns are both costly and time-consuming. It becomes especially complex to maintain an assurance case for a system when the requirements of the System-Under-Assurance change, or an assurance claim becomes invalid due to, e.g., degradation of a systems component, as common when deploying learning-enabled components. In this paper, we report on our preliminary experience leveraging the tool integration framework Evidential Tool Bus (ETB) for the construction and continuous maintenance of an assurance case from a predefined assurance case pattern. Specifically, we demonstrate the assurance process on an industrial Automated Valet Parking system from the automotive domain. We present the formalization of the provided assurance case pattern in the ETB processable logical specification language of workflows. Our findings show that ETB is able to create and maintain evidence required for the construction of an assurance case.

==> Sections/S3_Preliminaries.tex <==
\section{Preliminaries}
\label{Sec:Preliminaries}
\subsection{Assurance case}
Assurance case is a compelling, comprehensive, defensible, and valid justification of the system safety for a given application in a defined operating environment \cite{bishop2000methodology}; it is, therefore, a means to provide the grounds for confidence and to assist decision-making in certification \cite{bloomfield2009safety}. For decades, safety cases have been widely used in the European safety community to assure system safety. Moreover, they are mandatory in the regulation for systems used in safety-critical industries in some countries, e.g., in the UK for nuclear energy. Early research in safety cases has mainly focused on their formulation in terms of claims, arguments, and evidence elements based on fundamental argumentation theories like the Toulmin model \cite{toulmin2003uses}. The two most popular notations are Goal Structuring Notation (GSN) and Claims, Arguments, and Evidence (CAE). In this paper, we choose the former to present the assurance cases.



DSA \cite{DenneyDSC15} is required in scenarios such as when the requirements of the system-under-assurance (SUA) undergo modifications, or an assurance claim becomes invalid due to, e.g., degradation of a systems’ component. DSA is considered as a synergy between the design-time assurance case and runtime assurance. Thus, safety assurance is provided not only during initial development and deployment but also at runtime. The intent is to transform safety assurance into a continuous, evolutionary activity.   



\subsection{Evidential Tool Bus} ETB \footnote{\url{https://git.fortiss.org/etb2/etb2}} is a framework for defining and executing distributed assurance workflows that produce claims supported by evidence. \ETB enables an end-to-end, decentralized, and continuous safety assurance process where multiple entities are involved to establish safety claims supported by evidence. \ETB uses Datalog program as the assurance workflow scripting language and provides service wrappers to invoke external tools. The Datalog rules and wrappers form the assurance workflow, allowing for the argument to be initialized automatically, and rerunning the workflow as changes require, or simply to satisfy a skeptic or certification authorities. 


==> Sections/S5_Method.tex <==
\section{The Assurance Process}
\label{Sec:Methodology}

In this section, we describe the proposed assurance process along with its cornerstone concepts of distributed creation and continuous maintenance of assurance cases. 


\subsection{Assurance Framework: Evidential Tool Bus (ETB)} \ETB\footnote{\url{https://git.fortiss.org/etb2/etb2}} is a framework for defining and executing distributed assurance workflows that produce claims supported by evidence. \ETB enables an end-to-end, decentralized, and continuous safety assurance process where multiple entities are involved to establish safety claims supported by evidence. \ETB uses Datalog program as the assurance workflow scripting language and provides service wrappers to invoke external tools. The Datalog rules and wrappers form the assurance workflow, allowing for the argument to be initialized automatically, and rerunning the workflow as changes require, or simply to satisfy a skeptic or certification authorities. 

%% SECTION: Assurance Process
\subsection{Steps of the Assurance Process}
\label{Sec:SafetyAssurance}

The assurance process takes a top-level assurance goal as its input.
% , which is given in Fig.~\ref{fig:Methodology},
The assurance process consists of the following four steps: \textit{Assurance Pattern Creation}, \textit{Argument Pattern Formalisation}, \textit{Parameterisation of \ETB}, and \textit{Automated Assurance Case Creation}.
%
We illustrate these assurance steps using the \AVP system as a running example. 

\iffalse
%
\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.6]{Fig/Methodology.pdf}
    \caption{The proposed assurance methodology}
    \label{fig:Methodology}
\end{figure}
%
\fi

%% SUBSECTION: Assurance Pattern Creation
\subsubsection{Assurance Pattern Creation for the AVP System}

Let us consider a top-level assurance goal for the AVP system that claims \textit{``Whenever the vehicle bounding box intersects with the 3D bounding box of the pedestrian, the velocity of the vehicle is always 0"}.
%
While the objective here is not to develop a complete assurance case for the entire system, we present three argument patterns for the different abstraction levels of the system w.r.t the given safety goal. 
%
% We label this assurance goal as $\goal_1$.   
%
\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.47]{Fig/TopLevelAssurPattern.pdf}
    \caption{Top-level Assurance Pattern for the \AVP system}
    \label{fig:TopLevelAssurPattern}
\end{figure}
%
The first argument pattern, which is shown in Fig.~\ref{fig:TopLevelAssurPattern}, divides the top-level goal, which is labeled as $\goal_1$, into three sub-goals, $\goal_2$, $\goal_3$ and $\goal_4$, where $\goal_2$ targets the validation of the input requirements, and, $\goal_3$ and $\goal_4$ target the safety of the individual components and the overall system, respectively. 
%

The second argument pattern is dedicated to composing assurance arguments from each component of the \AVP system. 
As shown in Fig.~\ref{fig:ComponentsAssurPattern}, its three sub-goals, $\goal_8$, $\goal_9$ and $\goal_{10}$, target Object Detection (OD), Planning, and Control components of the \AVP system.  
%
\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.5]{Fig/ComponentsAssurPattern.pdf}
    \caption{Assurance Pattern over Components of the AVP system}
    \label{fig:ComponentsAssurPattern}
\end{figure}
%
%




The third argument pattern targets the OD component. Various recent approaches for the safety assurance of Learning-Enabled Components (LECs)\cite{hawkins2021guidance, wozniak2020safety,schwalbe2020structuring} propose safety assurance patterns over the LECs life-cycle. Building on such approaches, our argument pattern for the OD component targets data assurance, model assurance, verification assurance, and run-time assurance. 
%

\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.6]{Fig/ODAssurPattern.pdf}
    \caption{Assurance Pattern for the Object Detection Component}
    \label{fig:ODAssurPattern}
\end{figure}

As shown in Fig.~\ref{fig:ODAssurPattern}, its sub-goals, $\goal_{14}$, $\goal_{15}$, $\goal_{16}$ and $\goal_{17}$, target design-time (data, model and verification) and run-time assurance methods and evidence for the OD component.

%The three argument patterns illustrate how different strategies can be applied to construct assurance patterns for the AVP system at various granularity levels. 
%
The three argument patterns illustrate how assurance patterns can be constructed for the \AVP system at different granularity levels by applying appropriate strategies. 

\subsubsection{Formalisation of Assurance Argument Patterns}

%At the heart of our process is the \ETB framework, which is used for the creation and incremental maintenance of assurance cases for the \AVP system w.r.t the target goal. 
%\ETB requires assurance argument patterns to be specified in its scripting language of Datalog and all services, including formal and semi-formal verification and testing tools as well as human oracles, to be made available to it. 
%
As \ETB forms the crux of our assurance process, 
the developed argument patterns should be specified in Datalog, which is the scripting language of \ETB. 
For example, the top-level argument pattern (see Fig.~\ref{fig:TopLevelAssurPattern}) is formalised using 
Datalog program that is given below (Fig. \ref{Fig:DLAssurArg}). The head predicate is the top-level goal $\goal_1$, and its body contains each sub-goal of the argument pattern as a conjunct. 

\lstset{style=smallFrame}
%
\begin{figure}[!h]
    \centering
    \begin{lstlisting}[label=datalog1] 
g1_safe_AVP(SUA, Reqs, ODD, Datasets,   Specs,  RepSafEv,
      RepRelAss, ConfScore, CrTestCases, CSMRes, MERes) :-
    subcomponents(SUA, [OD, PC, CC]),
    g2_reqs(Reqs, Specs),
    g3_safe_components(SUA, ODD, Datasets,  Specs, RepSafEv, RepRelAss, ConfScore),
    g4_safe_system(SUA, Specs, Scenarios, CrTestCases, CSMRes, MERes).
\end{lstlisting}
\caption{A Datalog formalization of the example assurance argument}
    \label{Fig:DLAssurArg}
\end{figure}
%



%
%\begin{figure*}[t]
%    \centering
%    \includegraphics[scale=0.5]{Fig/AssuranceArgumentPatternOD.pdf}
%    \caption{Assurance case fragment for OD component.}
%    \label{Fig:SafetyCaseOD}
%\end{figure*}
%

Note that the goal predicates in the Datalog rule contain all the variables the goal depends on and a descriptive identifier, not just a goal index like the case for the assurance pattern. 
For instance, $\goal_1$ in the assurance pattern is now formalized as the following Datalog predicate.
\begin{equation*} \label{}
\begin{split}
g1&\_safe\_AVP  (SUA, Reqs, ODD, Datasets, Specs, \\ 
            & RepSafEv, RepRelAss, ConfScore, CrTestCases, \\
            & CSMRes, MERes)\\
\end{split}
\end{equation*}

In this predicate, the string $``safe\_AVP"$ is a descriptive post-fix of the goal name, and the parameters consist of the inputs such as \SUA, $Reqs$, ODD, and Datasets as well as resulting evidence artefacts like $CrTestCases$, which is a set of considered to be critical test cases identified by the system-level testing method. 
%\locTodo{Example specific input and outputs with formats}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Subsection: Integration of V&V Tools in ETB
\subsubsection{Integration of V\&V Tools in \ETB}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this step, tools that provide evidence artefacts during the actual creation of assurance cases are integrated into the \ETB framework. 
Following the common practice in tool integration frameworks, such as Jenkins~\footnote{https://www.jenkins.io/}, \ETB provides a wrappers API that auto-generates wrapper templates that can be customized by end-users for each tool. 
%This is a common practice in various tool integration framework such as Jenkins~\cite{}.
These wrappers are used to run tools, generate assurance evidence from the outputs of the tool executions, and attach a given evidence artefact with the corresponding low-level sub-goals in the target assurance case pattern. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Subsection: Automated Safety Case Creation
\subsubsection{Automated Safety Case Creation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The assurance case can be regarded as an instantiation of the assurance argument patterns. By utilizing the Datalog workflow, an assurance case construction can be seen as a collection of artifacts along with claims about these artifacts, and arguments in support of these claims. 

The ETB framework provides a top-down left-to-right Datalog engine that automatically executes the assurance workflow and also employs tools to create claims supported by evidence. 
By the end of the execution of the assurance workflow, ETB returns either a newly created assurance case or a counter-example that points to the failed step (sub-goal or tool execution) of the assurance process. The established claims, sub-claims, and evidence, which compose the assurance case for the AVP system, are given in Fig. \ref{fig:SafetyCaseAVP}. 
As clearly highlighted in the figure, the created claims can be categorised into two classes, namely high-level claims and low-level claims. 
While high-level claims correspond to the goals in the argument patterns that are supported by a set of sub-claims and a connecting argument, low-level claims are directly supported by evidence artifacts. 
ETB provides stores all these claims in the claims table and keeps track of all relevant tools and workflows w.r.t a given claim. 

\begin{figure} [!h]
    \centering
    \includegraphics[scale=0.30]{Fig/SafetyCaseAVP.png}
    \caption{Claims table that includes the generated claims, sub-claims, and assurance evidence.}
    \label{fig:SafetyCaseAVP}
\end{figure}

The claims can then be represented using traditional GSN-like assurance case notation. Fig. \ref{fig:GSNLikeRep} illustrates a GSN-like representation of the assurance case of the \AVP system.  

\begin{figure} [!h]
    \centering
    \includegraphics[scale=0.38]{Fig/GSNLike Assurance case AVP.png}
    \caption{GSN-Like representation of the claims table.}
    \label{fig:GSNLikeRep}
\end{figure}




%The automated safety case creation using \ETB is performed by executing the assurance workflow, specified as Datalog, and generating the claims, sub-claims, and assurance evidence. \ETB has a Datalog engine that executes the Datalog programs and invokes the verification tools to generate the assurance evidence. Indeed, some Datalog predicates are grounded using the outputs of the verification tools, this is done via services and wrappers, where \ETB invokes automatically these verification tools and associates the generated artifacts with the corresponding claims/sub-claims. 



%By the end of the execution of the Datalog program, \ETB returns either a newly created assurance case or a counter-example that points to the failed step (sub-goal or tool execution) of the assurance process. All the claims, sub-claims, and assurance evidence that compose the assurance case are stored in claims and evidence databases. The set of generated claims, sub-claims, and evidence can then be represented as GSN.




%We consider the assurance case fragment for OD illustrated in Fig. \ref{Fig:SafetyCaseOD}, starting from system-level requirement \textit{Safe\_AVP}, we obtain the core requirement for OD component \textit{Safe\_OD} illustrated in goal $\goal_{08}$, where \textit{``safe\_OD: OD component detects pedestrian with error tolerance of X given the ODD"}. This shall be achieved over the CE process i.e., design time by ensuring that OD is safe and reliable w.r.t \textit{safe\_OD} and runtime by ensuring that no undesired behavior of OD will appear in operation w.r.t \textit{safe\_OD}. 

%During design time, goal $\goal_{14}$, we ensure that the data used for the development of OD is sufficient and we conduct systematic testing to ensure the safety of OD against \textit{safe\_OD}, this is done by identifying and mitigating all safety threats leading to violation of \textit{safe\_OD}. The output of the systematic testing is a testing report recording how well the OD fulfills this requirement. In addition, we conduct additional verification to ensure that potential failures are acceptably managed by the OD model given the ODD.  During runtime, goal $\goal_{15}$, we applied runtime monitors to check the property of temporal consistency (i.e., reliability) of the OD. In addition, neuron activation monitoring (goal $\goal_{18}$) is applied to ensure the OD decisions are backed by prior similarities.   




%%%% SUBSECTION: Dynamic and Incremental Assurance
\subsection{Dynamic and Incremental Assurance} 
\label{subsec:DAC}

One defining feature of the proposed process is continuous assurance where updates to the \SUA, its requirements, or verification plans are anticipated.
In the event of such updates, outdated assurance artefacts including assurance cases and evidence artefacts are incrementally maintained, i.e., only a minimal set of maintenance actions are identified and executed.
The \ETB framework enables such assurance process by continuously executing relevant Datalog programs for outdated assurance cases and by continuously invoking verification tools for outdated assurance artefacts. 
% As we have formalized the assurance case through Datalog Programs, the assurance case is continuously constructed.
%\locTodo{Here, the reasoning engine tries to derive all claims in the rules when a claim is not in the claim database. A regeneration is triggered when parameters of a claim are changed.}

Let us consider a top-level claim $g1\_safeAVP(SUA,$ \\ $Reqs, ODD, Datasets, Specs,  RepSafEv, RepRelAss, $ \\ $ConfScore, CrTestCases,CSMRes, MERes)$ created for our running example. 
Let us assume the system requirements, represented with the variable $Reqs$, are updated due to the discovery of new safety vulnerabilities. 
This is very common in continuous engineering practices. 
%
\begin{figure}
    \centering
    \includegraphics[scale=0.42]{Fig/impact-tree.pdf}
    \caption{Example illustrating the incremental maintenance procedure after changing  the \texttt{Reqs} variable.}
    %Impacted predicates after changing \texttt{Reqs} variable.
    \label{fig:impact-tree}
\end{figure}
%
\ETB applies its light-weight static dependency computation procedure to compute a sub-tree of the assurance case impacted by the update. 
The procedure is applied to the formalized assurance pattern that was executed during the establishment of the top-level claim. 
The procedure distinguishes between two types of goals: \textit{directly impacted goals} and \textit{indirectly impacted goals}.
%
Directly impacted goals, such as $\goal_1$, $\goal_2$, $\goal_6$ and $\goal_7$, which are marked in red in Fig. \ref{fig:impact-tree}, should always be re-run to re-establish their corresponding claims. 
However, indirectly impacted goals, which are marked in yellow, may not need re-running if the re-running of the directly impacted goals did not result in an update to their assurance artefact. 
%\locTodo{Brief discussion.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% SUBSECTION: Distributed Assurance
\subsection{Distributed Assurance}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Another defining feature of the proposed process is the distribution of the assurance process where the task of creating assurance case fragments as well as assurance evidence can be distributed among multiple entities.
%
The advantage of such a distributed approach is two-fold. 
On one hand, it takes advantage of diverse assurance case fragments that are created separately~\cite{mscOmar2020}. 
It is common for complex systems, like the \AVP systems, to have multiple components each of which has unique engineering and assurance challenges. 
On the other hand, such a distributed process can take advantage of automated tools that can not be run on a common platform for creating assurance evidence. 
Certification standards across various domains, such as DO-178C in Avionics and ISO 26262 in Automotive, encourage the use of complementary tools when a single tool is not sufficient for a given test, analysis or verification activity. 

\iffalse
In this work, we consider two classes of arguments, namely \textit{Assurance Arguments} and \textit{Verification Arguments}. 
An Assurance Argument for a given high-level assurance goal defines a set of necessary and sufficient sub-goals that support the goal. 
For example, the assurance argument that results from instantiating the argument pattern in Fig.~\ref{fig:TopLevelAssurPattern} falls into the category of Assurance Arguments. 
%
The focus of Verification Arguments, on the other hand, is providing necessary and sufficient evidence, i.e., solutions in GSN terminology, for low-level goals. 
%
An example verification argument is shown in Figure~\ref{Fig:VerifArg}.
\locTodo{The argument defines that ... arg explain}. 
%
\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.9]{Fig/VerificationArgument.pdf}
    \caption{An example Verification Argument}
    \label{Fig:VerifArg}
\end{figure}
%

This separation of concern between assurance and verification arguments enables effective incremental maintenance by separating the localization of impacts due to changes to the assurance process inputs from the actual maintenance of affected evidence artefacts. 
%
For instance, if there is a newly identified safety threat and changes need to be made to the verification plan, the assurance arguments (together with all the unaffected higher-level safety claims) can stay the same, while the relevant verification argument needs an update to ensure a stronger evidence, that takes into considerations the new safety threat, is created.
%
Similarly, if one component is added to the \SUA, existing verification arguments can stay the same but the relevant assurance argument needs an update to ensure all system components are covered in the assurance argument. 
%
This will be explained further in Section~\ref{subsec:DAC}. 

The proposed methodology regards assurance case patterns as comprising a set of assurance and verification arguments, and developing the assurance case pattern is the first step of the methodology. 
As in the state-of-practice, this step is a manual effort since it involves domain knowledge and subjective reasoning. 
In the second step of the methodology, a given assurance case pattern is formalized in Datalog, which is the specification language of the \ETB framework. 
\locTodo{The formalized Datalog workflows for the example assurance (resp. verification) argument, which is shown in Figure~\ref{Fig:AssurArg} (Figure~\ref{Fig:VerifArg}), is given in Figure~\ref{Fig:DLAssurArg}.}
\fi

The use of \ETB enables the creation of both assurance cases and evidence artefacts by executing the Datalog workflows in a distributed setting. 
Practically, a network of \ETB nodes is defined where each node can create assurance cases or evidence artefacts depending on the type of workflow it contains. 
A given \ETB node provides a set of workflows and automated tools that can contribute to the overall assurance process that comprises multiple nodes. 



==> Sections/appendices.tex <==
\appendices
\newpage
\onecolumn
\section{Top-level Assurance Pattern}
\label{app:datalogWorkflow}


